ELEPHANT: ExtragaLactic alErt Pipeline for Hostless AstroNomical Transients

Context. Transient astronomical events that exhibit no discernible association with a host galaxy are commonly referred to as hostless. These rare phenomena are associated with extremely energetic events, and they can offer unique insights into the properties and evolution of stars and galaxies. However, the sheer number of transients captured by contemporary high-cadence astronomical surveys renders the manual identification of all potential hostless transients impractical. Therefore, creating a systematic identification tool is crucial for studying these elusive events. Aims. We present the ExtragaLactic alErt Pipeline for Hostless AstroNomical Transients (ELEPHANT), a framework for filtering hostless transients in astronomical data streams. Methods. We used Fink to access all the ZTF alerts produced between January/2022 and December/2023, selecting only those associated with extragalactic transients. We then processed the associated stamps using a sequence of image analysis techniques to retrieve hostless candidates. Results. We find that less than 2% of all analyzed transients are potentially hostless. Among them, approximately 10% have a spectroscopic class reported on TNS, with Type Ia supernova being the most common class, followed by SLSN. Among the hostless candidates retrieved by our pipeline, there was SN 2018ibb, which has been proposed to be a PISN candidate; and SN 2022ann, one of only five known SNe Icn. When no class is reported on TNS, the dominant classes are QSO and SN candidates, the former obtained from SIMBAD and the latter inferred using the Fink ML classifier. Conclusions. ELEPHANT represents an effective strategy to filter extragalactic events within large and complex astronomical alert streams. There are many applications for which this pipeline will be useful, ranging from transient selection for follow-up to studies of transient environments.

==> tex/plot_distance.tex <==
\begin{figure*}
    \includegraphics[width=1\textwidth]{figures/TempX2_distance.png}
  \caption{Right panel shows the \textcolor{red}{[science? template? first? last? co-added?]} stamp of the 60x60 region for the \textbf{X2} transient with log transformation. The left panel shows the masked regions (red) that correspond to one or more detected sources. The circumference has 7-pixel radius. We assume a single pixel in the centre of the image at position (30,30) to calculate the distance between the transient and its closest neighbour. In this figure, we see that its closest neighbor is at a diagonally adjacent pixel. }
\label{fig:distance}
\end{figure*}

==> tex/plot_hostless.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/sigma_clipping.png}
    \caption{Sigma clipping on science and template patches}
    \label{fig:sigma_clipping_fig}
\end{figure}


\begin{figure}
        \centering
        \includegraphics[width=0.5\linewidth]{figures/potential_hostless2.png}
    \centering

    \includegraphics[width=0.5\linewidth]{figures/potential_hostless1.png}
    \caption{Visual example of flagged hostless candidates}
    \label{fig:potential_hostless_examples}
\end{figure}

==> tex/plot_legacy.tex <==
\begin{figure*}

    \subfloat[(put here an example of a hostless transient)]
    % {\includegraphics[width=0.45\textwidth]{fig/distribution_train_test.png}}
{\includegraphics[width=1\textwidth]{figures/ZTF18aacibvx.png}}
    \label{fig:legacy_a}
    
    \subfloat[(put here an example of a transient with a host)]
    % {\includegraphics[width=0.45\textwidth]{fig/distribution_train_test_r.png}}
{\includegraphics[width=1\textwidth]{figures/ZTF18aafoaiy.png}}
\label{fig:legacy_b}

\caption{}

\label{fig:legacy}
\end{figure*}
